The Arf-Brown TQFT of Pin$^-$ Surfaces

The Arf-Brown invariant $\mathit{AB}(\Sigma)$ is an 8th root of unity associated to a surface $\Sigma$ equipped with a pin$^-$ structure. In this note we investigate a certain fully extended, invertible, topological quantum field theory (TQFT) whose partition function is the Arf-Brown invariant. Our motivation comes from the recent work of Freed-Hopkins on the classification of topological phases, of which the Arf-Brown TQFT provides a nice example of the general theory; physically, it can be thought of as the low energy effective theory of the Majorana chain, or as the anomaly theory of a free fermion in 1 dimension.

==> homotopy_fixed_points.tex <==
% idea, and cite who used this periodicity already
The $\Z/2$ classification of stable invertible 2D spin TQFTs and the $\Z/8$ classification in the \pinm case are
reminiscent of the $\Z/2$ and $\Z/8$ classifications of complex and real Clifford algebras up to Morita
equivalence. One might wonder whether these are ``the same'' $\Z/2$ and $\Z/8$ in both cases, i.e.\ whether these
isomorphisms are induced by some functor between Clifford algebras and TQFTs. In this section, we sketch an answer,
using the cobordism hypothesis to relate these two classifications.\todo{Rather than Clifford algebras, maybe the
Brauer-Wall groups of $\C$ and $\R$.}

This correspondence has been observed in a different setting in the theory of condensed-matter physics, where a
version of it is used to classify symmetry-protected topological (SPT) phases. Insights from physics tell us that,
conjecturally, there is a correspondence between certain kinds of 2D fermionic SPTs and deformation classes of 2D
spin and \pinm invertible TQFTs.\todo{Cite} (We'll say more about this in \S\ref{TR_Majorana}.) There are
different approaches to classifying these SPT phases, but those of Fidkowski-Kitaev~\cite{FK11} and
Gaiotto-Johnson-Freyd~\cite{GJF17} make explicit use of Brauer-Wall groups of $\C$ for spin phases, $\R$ for
\pinm phases, and $\H$ for \pinp phases.\footnote{Strictly speaking, superalgebra over $\H$ does not make sense;
the replacement is to work with algebras whose even components are real and whose odd components are quaternionic.}

\dots % much work to be done

% first part: argument in the spin case, which is fully understood



% second part: argument in the pin^- case, which is less understood...

